Identifying the Best Transition Law

Motivated by recursive learning in Markov Decision Processes, this paper studies best-arm identification in bandit problems where each arm's reward is drawn from a multinomial distribution with a known support. We compare the performance { reached by strategies including notably LUCB without and with use of this knowledge. } In the first case, we use classical non-parametric approaches for the confidence intervals. In the second case, where a probability distribution is to be estimated, we first use classical deviation bounds (Hoeffding and Bernstein) on each dimension independently, and then the Empirical Likelihood method (EL-LUCB) on the joint probability vector. The effectiveness of these methods is demonstrated through simulations on scenarios with varying levels of structural complexity.

==> JSC_def.tex <==
\newcommand{\bs}{\boldsymbol}
\newcommand{\mc}{\mathcal}

\newcommand{\cond}{\,\vert\,}
\newcommand{\Qxh}{Q_{x|h}}
\newcommand{\QxhW}{Q_{x|hW}}
\newcommand{\defeq}{\triangleq}
\newcommand{\defeqd}{\stackrel{\text{def}}{=}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\xh}{{\bar{x}_h}}
\newcommand{\xhW}{{\bar{x}_{hW}}}
\newcommand{\xhi}{{\bar{x}_{h,i}}}
\newcommand{\xhWi}{{\bar{x}_{hW,i}}}
\newcommand{\T}{{\scriptscriptstyle\mathsf{T}}}
\renewcommand{\H}{{\scriptscriptstyle\mathsf{H}}}
%\newcommand{\Cov}{{\mathsf{Cov}}}
\newcommand{\Prr}{\textnormal{Pr}}

% bb font symbols

\newfont{\bbb}{msbm10 scaled 500}
\newcommand{\CCC}{\mbox{\bbb C}}

\newfont{\bb}{msbm10 scaled 1100}
\newcommand{\CC}{\mbox{\bb C}}
\newcommand{\RR}{\mbox{\bb R}}
\newcommand{\ZZ}{\mbox{\bb Z}}
\newcommand{\FF}{\mbox{\bb F}}
\newcommand{\GG}{\mbox{\bb G}}
%\newcommand{\EE}{\mathbb{E}}
\newcommand{\NN}{\mbox{\bb N}}

% Vectors

\newcommand{\av}{{\bf a}}
\newcommand{\bv}{{\bf b}}
\newcommand{\cv}{{\bf c}}
\newcommand{\dv}{{\bf d}}
\newcommand{\ev}{{\bf e}}
\newcommand{\fv}{{\bf f}}
\newcommand{\gv}{{\bf g}}
\newcommand{\hv}{{\bf h}}
\newcommand{\iv}{{\bf i}}
\newcommand{\jv}{{\bf j}}
\newcommand{\kv}{{\bf k}}
\newcommand{\lv}{{\bf l}}
\newcommand{\mv}{{\bf m}}
\newcommand{\nv}{{\bf n}}
\newcommand{\ov}{{\bf o}}
\newcommand{\pv}{{\bf p}}
\newcommand{\qv}{{\bf q}}
\newcommand{\rv}{{\bf r}}
\newcommand{\sv}{{\bf s}}
\newcommand{\tv}{{\bf t}}
\newcommand{\uv}{{\bf u}}
\newcommand{\wv}{{\bf w}}
\newcommand{\vv}{{\bf v}}
\newcommand{\xv}{{\bf x}}
\newcommand{\yv}{{\bf y}}
\newcommand{\zv}{{\bf z}}
\newcommand{\zerov}{{\bf 0}}
\newcommand{\onev}{{\bf 1}}

% Matrices

\newcommand{\Am}{{\bf A}}
\newcommand{\Bm}{{\bf B}}
\newcommand{\Cm}{{\bf C}}
\newcommand{\Dm}{{\bf D}}
\newcommand{\Em}{{\bf E}}
\newcommand{\Fm}{{\bf F}}
\newcommand{\Gm}{{\bf G}}
\newcommand{\Hm}{{\bf H}}
\newcommand{\Id}{{\bf I}}
\newcommand{\Jm}{{\bf J}}
\newcommand{\Km}{{\bf K}}
\newcommand{\Lm}{{\bf L}}
\newcommand{\Mm}{{\bf M}}
\newcommand{\Nm}{{\bf N}}
\newcommand{\Om}{{\bf O}}
\newcommand{\Pm}{{\bf P}}
\newcommand{\Qm}{{\bf Q}}
\newcommand{\Rm}{{\bf R}}
\newcommand{\Sm}{{\bf S}}
\newcommand{\Tm}{{\bf T}}
\newcommand{\Um}{{\bf U}}
\newcommand{\Wm}{{\bf W}}
\newcommand{\Vm}{{\bf V}}
\newcommand{\Xm}{{\bf X}}
\newcommand{\Ym}{{\bf Y}}
\newcommand{\Zm}{{\bf Z}}

% Calligraphic

\newcommand{\Ac}{{\cal A}}
\newcommand{\ac}{{\cal a}}
\newcommand{\Bc}{{\cal B}}
\newcommand{\CDc}{{\cal{CD}}}
\newcommand{\Cc}{{\cal C}}
\newcommand{\Dc}{{\cal D}}
\newcommand{\Ec}{{\cal E}}
\newcommand{\Fc}{{\cal F}}
\newcommand{\Gc}{{\cal G}}
\newcommand{\Hc}{{\cal H}}
\newcommand{\Ic}{{\cal I}}
\newcommand{\Jc}{{\cal J}}
\newcommand{\Kc}{{\cal K}}
\newcommand{\Lc}{{\cal L}}
\newcommand{\Mc}{{\cal M}}
\newcommand{\Nc}{{\cal N}}
\newcommand{\Oc}{{\cal O}}
\newcommand{\Pc}{{\cal P}}
\newcommand{\Qc}{{\cal Q}}
\newcommand{\Rc}{{\cal R}}
\newcommand{\Sc}{{\cal S}}
\newcommand{\Tc}{{\cal T}}
\newcommand{\Uc}{{\cal U}}
\newcommand{\Wc}{{\cal W}}
\newcommand{\Vc}{{\cal V}}
\newcommand{\Xc}{{\cal X}}
\newcommand{\Yc}{{\cal Y}}
\newcommand{\Zc}{{\cal Z}}


\newcommand{\tT}{{\tilde T}}


% Bold greek letters

\newcommand{\alphav}{\hbox{\boldmath$\alpha$}}
\newcommand{\betav}{\hbox{\boldmath$\beta$}}
\newcommand{\gammav}{\hbox{\boldmath$\gamma$}}
\newcommand{\deltav}{\hbox{\boldmath$\delta$}}
\newcommand{\etav}{\hbox{\boldmath$\eta$}}
\newcommand{\lambdav}{\hbox{\boldmath$\lambda$}}
\newcommand{\epsilonv}{\hbox{\boldmath$\epsilon$}}
\newcommand{\nuv}{\hbox{\boldmath$\nu$}}
\newcommand{\muv}{\hbox{\boldmath$\mu$}}
\newcommand{\zetav}{\hbox{\boldmath$\zeta$}}
\newcommand{\phiv}{\hbox{\boldmath$\phi$}}
\newcommand{\psiv}{\hbox{\boldmath$\psi$}}
\newcommand{\thetav}{\hbox{\boldmath$\theta$}}
\newcommand{\tauv}{\hbox{\boldmath$\tau$}}
\newcommand{\omegav}{\hbox{\boldmath$\omega$}}
\newcommand{\xiv}{\hbox{\boldmath$\xi$}}
\newcommand{\sigmav}{\hbox{\boldmath$\sigma$}}
\newcommand{\piv}{\hbox{\boldmath$\pi$}}
\newcommand{\rhov}{\hbox{\boldmath$\rho$}}
\newcommand{\Gammam}{\hbox{\boldmath$\Gamma$}}
\newcommand{\Lambdam}{\hbox{\boldmath$\Lambda$}}
\newcommand{\Deltam}{\hbox{\boldmath$\Delta$}}
\newcommand{\Sigmam}{\hbox{\boldmath$\Sigma$}}
\newcommand{\Phim}{\hbox{\boldmath$\Phi$}}
\newcommand{\Pim}{\hbox{\boldmath$\Pi$}}
\newcommand{\Psim}{\hbox{\boldmath$\Psi$}}
\newcommand{\Thetam}{\hbox{\boldmath$\Theta$}}
\newcommand{\Omegam}{\hbox{\boldmath$\Omega$}}
\newcommand{\Xim}{\hbox{\boldmath$\Xi$}}

%{% mixed symbols
%\newcommand{\sinc}{{\hbox{sinc}}}
%\newcommand{\diag}{{\hbox{diag}}}
%\renewcommand{\det}{{\hbox{det}}}
%\newcommand{\trace}{{\hbox{tr}}}
%\newcommand{\rank}{{\hbox{rank}}}
%\newcommand{\sign}{{\hbox{sign}}}
%\renewcommand{\arg}{{\hbox{arg}}}
\newcommand{\var}{{\hbox{var}}}
%\newcommand{\SINR}{{\sf SINR}}
%%\newcommand{\SNR}{{\sf SNR}}
%\newcommand{\SIR}{{\sf SIR}}
%\newcommand{\Ei}{{\rm E}_{\rm i}}
%\renewcommand{\Re}{{\rm Re}}
%\renewcommand{\Im}{{\rm Im}}
%\newcommand{\eqdef}{\stackrel{\Delta}{=}}
%\newcommand{\defines}{{\,\,\stackrel{\scriptscriptstyle \bigtriangleup}{=}\,\,}}
%\newcommand{\<}{\left\langle}
%\renewcommand{\>}{\right\rangle}
%\newcommand{\cov}{{\hbox{cov}}} 
%%
%\newcommand{\dis}{{ \text{d}}}
%\newcommand{\Pro}{{ \text{P}}}
%\newcommand{\tT}{{ \tilde{T}}}
%\newcommand{\tZ}{{ \tilde{Z}}}
%\newcommand{\tY}{{ Z}}
%%
%\DeclareFontFamily{U}{cmfi}{}
%\DeclareFontShape{U}{cmfi}{m}{n}{ <-> cmfi10 }{}
%\DeclareSymbolFont{CMFI}{U}{cmfi}{m}{n}
%\def\expect{\mathop{{\rm E}}}

%\newcommand{\e}[1]{{\rm e}^{#1}}
%\newcommand{\e}{{\rm e}}
%
%\newcommand{\define}{\stackrel{\triangle}{=}}
%\def\mathlette#1#2{{\mathchoice{\mbox{#1$\displaystyle #2$}}%
%		{\mbox{#1$\textstyle #2$}}%
%		{\mbox{#1$\scriptstyle #2$}}%
%		{\mbox{#1$\scriptscriptstyle #2$}}}}
%\newcommand{\matr}[1]{\mathlette{\boldmath}{#1}}
%\def\argmax{\mathop{\rm argmax}}
% limits underneath
%\newcommand{\argmax}[2]{\operatorname*{arg\,max}_{#1} #2}
%\newcommand{\argmin}[2]{\operatorname*{arg\,min}_{#1} #2}

%
%\newcommand{\eq}[1]{(\ref{#1})}
%\newcommand{\Ts}{T_{\rm s}}


\newcommand{\vh}{\pmb{h}}
\newcommand{\vg}{\pmb{g}}
\newcommand{\vx}{\pmb{x}}
\newcommand{\vz}{\pmb{z}}
\newcommand{\vy}{\pmb{y}}
\newcommand{\vu}{\pmb{u}}
\renewcommand{\vv}{\pmb{v}}
\newcommand{\vb}{\pmb{b}}
\newcommand{\ve}{\pmb{e}}


%% \newcommand{\rvh}{H}
%% \newcommand{\rvg}{G}
%% \newcommand{\rvx}{X}
%% \newcommand{\rvz}{Z}
%% \newcommand{\rvy}{Y}
%% \newcommand{\rvu}{U}
%% \newcommand{\rvv}{V}
%% \newcommand{\rvb}{B}
%% \newcommand{\rve}{E}
%% 
%% \newcommand{\rh}{H}
%% \newcommand{\rg}{G}
%% \newcommand{\rx}{X}
%% \newcommand{\rvz}{Z}
%% \newcommand{\rvy}{Y}
%% \newcommand{\ru}{U}
%% \renewcommand{\rv}{V}
%% \newcommand{\rb}{B}
%\newcommand{\snr}{\mathsf{snr}}
%\newcommand{\SNR}{\mathsf{snr}}
%\newcommand{\DoF}{\mathsf{DoF}}
%\newcommand{\taulog}{\mathit{o}(\log \snr)}

\newcommand{\vA}{\vv_{\A}}
\newcommand{\vB}{\vv_{\B}}

\newcommand{\nA}{n_{\A}}
\newcommand{\nB}{n_{\B}}

\newcommand{\mA}{m_{\A}}
\newcommand{\mB}{m_{\B}}


\newcommand{\dA}{d_{\A}}
\newcommand{\dB}{d_{\B}}

\newcommand{\MA}{M_{\A}}
\newcommand{\MB}{M_{\B}}




%% %%random scalars
%% \newcommand{\rvW}{{\mathsf{W}}}
%% \newcommand{\rvx}{{\mathsf{x}}}
%% \newcommand{\rvy}{{\mathsf{y}}}
%% \newcommand{\rvz}{{\mathsf{z}}}
%% %%random vectors
%% \newcommand{\rvU}{\pmb{\mathsf{u}}}
%% \newcommand{\rvV}{\pmb{\mathsf{v}}}
%% \newcommand{\rvE}{\pmb{\mathsf{e}}}
%% \newcommand{\rvY}{\pmb{\mathsf{y}}}
%% \newcommand{\rvZ}{\pmb{\mathsf{z}}}
%% \newcommand{\rvX}{\pmb{\mathsf{x}}}
%% \newcommand{\rvB}{\pmb{\mathsf{b}}}
%% %%random matrices
%% \newcommand{\rvH}{\pmb{\mathsf{H}}}
%% \newcommand{\rvG}{\pmb{\mathsf{G}}}
%% 
%%random scalars
\newcommand{\rvW}{{{W}}}
\newcommand{\rvx}{{{x}}}
\newcommand{\rvy}{{{y}}}
\newcommand{\rvz}{{{z}}}
%%random vectors
\newcommand{\rvU}{\pmb{{u}}}
\newcommand{\rvV}{\pmb{{v}}}
\newcommand{\rvE}{\pmb{{e}}}
\newcommand{\rvY}{\pmb{{y}}}
\newcommand{\rvZ}{\pmb{{z}}}
\newcommand{\rvX}{\pmb{{x}}}
\newcommand{\rvB}{\pmb{{b}}}
%%random matrices
\newcommand{\rvH}{\pmb{{H}}}
\newcommand{\rvG}{\pmb{{G}}}

\renewcommand{\Thetam}{ {\bf{{\Theta}}}}
\newcommand{\ThetamA}{\Thetam_{{\A}}}
\newcommand{\ThetamB}{\Thetam_{{\B}}}
\renewcommand{\Phim}{ {\bf{{\Phi}}} }
\newcommand{\PhimA}{\Phim_{{\A}}}
\newcommand{\PhimB}{\Phim_{{\B}}}

%\newcommand{\He}{\pmb{\mathsf{\widehat{H}}}}
\newcommand{\He}{\pmb{{\mathrm{\hat{H}}}}}
%\newcommand{\Ge}{\pmb{\mathsf{\widehat{G}}}}
\newcommand{\Ge}{\pmb{{\mathrm{\hat{G}}}}}

\newcommand{\WA}{\rvW_{\A}}



\newcommand{\WB}{\rvW_{\B}}
\newcommand{\WAhat}{\hat{\rvW}_{\A}}
\newcommand{\WBhat}{\hat{\rvW}_{\B}}
\newcommand{\dotle}{\ \dot{\le}\  }
\newcommand{\dotge}{\ \dot{\ge}\  }

\renewcommand{\Am}{\pmb{A}}
\renewcommand{\Bm}{\pmb{B}}
\renewcommand{\Cm}{\pmb{C}}
\renewcommand{\Dm}{\pmb{D}}
\renewcommand{\Em}{\pmb{E}}
\renewcommand{\Fm}{\pmb{F}}
\renewcommand{\Gm}{\pmb{G}}
\renewcommand{\Hm}{\pmb{H}}
\renewcommand{\Jm}{\pmb{J}}
\renewcommand{\Km}{\pmb{K}}
\renewcommand{\Lm}{\pmb{L}}
\renewcommand{\Mm}{\pmb{M}}
\renewcommand{\Nm}{\pmb{N}}
\renewcommand{\Om}{\pmb{O}}
\renewcommand{\Pm}{\pmb{P}}
\renewcommand{\Qm}{\pmb{Q}}
\renewcommand{\Rm}{\pmb{R}}
\renewcommand{\Sm}{\pmb{S}}
\renewcommand{\Tm}{\pmb{T}}
\renewcommand{\Um}{\pmb{U}}
\renewcommand{\Vm}{\pmb{V}}
\renewcommand{\Wm}{\pmb{W}}
\renewcommand{\Xm}{\pmb{X}}
\renewcommand{\Ym}{\pmb{Y}}
\renewcommand{\Zm}{\pmb{Z}}

\renewcommand{\av}{\pmb{a}}
\renewcommand{\bv}{\pmb{b}}
\renewcommand{\cv}{\pmb{c}}
\renewcommand{\dv}{\pmb{d}}
\renewcommand{\ev}{\pmb{e}}
\renewcommand{\fv}{\pmb{f}}
\renewcommand{\gv}{\pmb{g}}
\renewcommand{\hv}{\pmb{h}}
\renewcommand{\jv}{\pmb{j}}
\renewcommand{\kv}{\pmb{k}}
\renewcommand{\lv}{\pmb{l}}
\renewcommand{\mv}{\pmb{m}}
\renewcommand{\nv}{\pmb{n}}
\renewcommand{\ov}{\pmb{o}}
\renewcommand{\pv}{\pmb{p}}
\renewcommand{\qv}{\pmb{q}}
\renewcommand{\rv}{\pmb{r}}
\renewcommand{\sv}{\pmb{s}}
\renewcommand{\tv}{\pmb{t}}
\renewcommand{\uv}{\pmb{u}}
\renewcommand{\vv}{\pmb{v}}
\renewcommand{\wv}{\pmb{w}}
\renewcommand{\xv}{\pmb{x}}
\renewcommand{\yv}{\pmb{y}}
\renewcommand{\zv}{\pmb{z}}

% Colors

\newcommand{\RED}{\color[rgb]{1.00,0.10,0.10}}
\newcommand{\BLUE}{\color[rgb]{0,0,0.90}}
\newcommand{\GREEN}{\color[rgb]{0,0.80,0.20}}
% Markov chain
\newcommand{\mkv}{-\!\!\!\!\minuso\!\!\!\!-}

\newcommand{\gp}[1]{{#1}}

%Defining Symbols to be used 
\newcommand{\ind}[1]{\mathds{1}_{\left\lbrace #1 \right\rbrace}}
%\newcommand{\norm}[1]{\left|\left| #1 \right|\right|}
\newcommand{\bigO}[1]{\ensuremath{\mathop{}\mathopen{}O\mathopen{}\left(#1\right)}}
\newcommand{\smallO}[1]{\ensuremath{\mathop{}\mathopen{}o\mathopen{}\left(#1\right)}}
